On the Complexity of Rearrangement Problems under the Breakpoint Distance

We study complexity of rearrangement problems in the generalized breakpoint model and settle several open questions. The model was introduced by Tannier et al. (2009) who showed that the median problem is solvable in polynomial time in the multichromosomal circular and mixed breakpoint models. This is intriguing, since in most other rearrangement models (DCJ, reversal, unichromosomal or multilinear breakpoint models), the problem is NP-hard. The complexity of the small or even the large phylogeny problem under the breakpoint distance remained an open problem. We improve the algorithm for the median problem and show that it is equivalent to the problem of finding maximum cardinality non-bipartite matching (under linear reduction). On the other hand, we prove that the more general small phylogeny problem is NP-hard. Surprisingly, we show that it is already NP-hard (or even APX-hard) for 4 species (a quartet phylogeny). In other words, while finding an ancestor for 3 species is easy, finding two ancestors for 4 species is already hard. We also show that, in the unichromosomal and the multilinear breakpoint model, the halving problem is NP-hard, thus refuting the conjecture of Tannier et al. Interestingly, this is the first problem which is harder in the breakpoint model than in the DCJ or reversal models.

==> Makefile <==
all: main.pdf

clean:
	-rm main.aux main.bbl main.blg main.log main.log main.lot main.out \
	main.dvi main.ps main.pdf *~

main.ps: main.dvi
	dvips main -o main.ps

main.pdf:  main.tex *.tex *.bib figs/*.pdf
	pdflatex main
	pdflatex main
	-bibtex main
	pdflatex main
	pdflatex main


main.dvi:  main.tex *.tex *.bib
	latex main
	latex main
	-bibtex main
	latex main
	latex main


